The Power Spectrum of Climate Change

Both global, intermediate and local scales of Climate Change have been studied extensively, but a unified diagnostic framework for examining all spatial scales concurrently has remained elusive. Here we present a new tool-set using spherical harmonics to examine climate change through surface temperature anomalies from 1850 to 2021 on spatial scales ranging from planetary to $50$ km scales. We show that the observed temperature anomalies are accurately decomposed in spherical harmonics typically within 0.05 K. This decomposition displays a remarkably simple dependence on spatial scale with a universal shape across seasons and decades. The decomposition separates two distinct regimes by a characteristic turnover-length of approximately $3000$ km. The largest scales confirm established trends, while local fluctuations are consistent with 2-dimensional turbulence. We observe a downward cascade, from which it follows that climate change feeds increasing volatility on all spatial scales from $2.000$ to $50$ km. This increase is primarily driven by growing volatility along longitudes.

==> trash.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{r_present_corr_coef_2.png}
         \caption{Correlation Coefficient between power of modes simultaneously. }
         \label{fig:corr_coeff}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{r_corr_coef_2.png}
         \caption{Correlation Coefficient between power of modes in neighbouring months.}
         \label{fig:corr_coeff}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{r_residual_2.png}
         \caption{The correlation between powers across subsequent months is not symmetric. There is more correlation between lower modes in previous months with larger modes in subsequent months then between larger modes in previous months with lower modes in ensuing months.}
         \label{fig:corr_coeff}
    \end{subfigure}
    \caption{Typically modes of similar spatial scales are more correlated while all modes within the cascade show large correlation. }
\end{figure}
